Deflation-based certified greedy algorithm and adaptivity for bifurcating nonlinear PDEs

This work deals with tailored reduced order models for bifurcating nonlinear parametric partial differential equations, where multiple coexisting solutions arise for a given parametric instance. Approaches based on proper orthogonal decomposition have been widely investigated in the literature, but they usually rely on some \emph{a-priori} knowledge about the bifurcating model and lack any error estimation. On the other hand, standard certified reduced basis techniques fail to represent correctly the branching behavior, since the error estimator is no longer reliable. The main goal of the contribution is to overcome these limitations by introducing two novel algorithms: (i) the adaptive-greedy, detecting the bifurcation point starting from scarce information over the parametric space, and (ii) the deflated-greedy, certifying multiple coexisting branches simultaneously. The former approach takes advantage of the features of the reduced manifold to detect the bifurcation, while the latter exploits the deflation and continuation methods to discover the bifurcating solutions and enrich the reduced space. We test the two strategies for the Coanda effect held by the Navier-Stokes equations in a sudden-expansion channel. The accuracy of the approach and the error certification are compared with vanilla-greedy and proper orthogonal decomposition.

==> sections/PODresults.tex <==
\section{Additional POD results (experiment 4)}
\label{app:PODresults}
This section shows some additional results of the POD applied to the numerical setting of Section \ref{sec:results}. We recall that we are performing a branch-wise POD over 51 equispaced parameters in $\mathcal P = [0.5, 2]$ and we retain the first $N=25$ modes.
\mari{fare un'unica figura con gli errori sommati? Come abbiamo fatto per il greedy? E magari mettere gli errori relativi che scendono e non scendono rispetto a N?} In Figure \ref{fig:PODrel_cert} we depict the relative error $E_{vp}$ and the projection errors for the symmetric, top asymmetric and bottom symmetric solutions, from left to right, respectively. We see that the POD is able to reconstruct only the symmetric branch, i.e. the one related to the snapshots collection. For this reason, the POD is not really suited for bifurcating phenomena without any knowledge of the system. Indeed, while the POD represents with no issue the pre-bifurcating behaviour, totally fails in representing solutions for $\mu \leq \mu^*=0.96$. 
\begin{figure}[H]
    \centering
\includegraphics[width=0.3\textwidth]{img/pod/RB_error_velocity_sym.png}
\includegraphics[width=0.3\textwidth]{img/pod/RB_error_velocity_asym.png}
\includegraphics[width=0.3\textwidth]{img/pod/RB_error_velocity_asym_lower.png}
\caption{Experiment 4: reduced and projection relative errors for the velocity field, symmetric, asymmetric top and asymmetric bottom, left to right respectively (N = 25).}
\label{fig:PODrel_cert}
\end{figure}


\begin{figure}[H]
    \centering
    \includegraphics[width=0.3\textwidth]{img/pod/RB_error_pressure_sym.png}
\includegraphics[width=0.3\textwidth]{img/pod/RB_error_pressure_asym.png}
\includegraphics[width=0.3\textwidth]{img/pod/RB_error_pressure_asym_lower.png}
\caption{Reduced and projection relative errors for the pressure field, symmetric, asymmetric top and asymmetric bottom, left to right respectively.}
\end{figure}

